Time-Window Group-Correlation Support vs. Individual Features: A Detection of Abnormal Users

Autoencoder-based anomaly detection methods have been used in identifying anomalous users from large-scale enterprise logs with the assumption that adversarial activities do not follow past habitual patterns. Most existing approaches typically build models by reconstructing single-day and individual-user behaviors. However, without capturing long-term signals and group-correlation signals, the models cannot identify low-signal yet long-lasting threats, and will wrongly report many normal users as anomalies on busy days, which, in turn, lead to high false positive rate. In this paper, we propose ACOBE, an Anomaly detection method based on COmpound BEhavior, which takes into consideration long-term patterns and group behaviors. ACOBE leverages a novel behavior representation and an ensemble of deep autoencoders and produces an ordered investigation list. Our evaluation shows that ACOBE outperforms prior work by a large margin in terms of precision and recall, and our case study demonstrates that ACOBE is applicable in practice for cyberattack detection.

==> plotfigures.tex <==

\begin{figure*}
\centering
\subfigure[r6.1 Scenario 1: Acobe (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-deviceg1_trends.png}
    \label{behfig:acobe:r1s1device.png}} 
\subfigure[r6.1 Scenario 1: Acobe (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-fileg1_trends.png}
    \label{behfig:acobe:r1s1file.png}} 
\subfigure[r6.1 Scenario 1: Acobe (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-httpg1_trends.png}
    \label{behfig:acobe:r1s1http.png}} 
    
\subfigure[r6.1 Scenario 1: egh (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-deviceg1_trends.png}
    \label{behfig:egh:r1s1device.png}} 
\subfigure[r6.1 Scenario 1: egh (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-fileg1_trends.png}
    \label{behfig:egh:r1s1file.png}} 
\subfigure[r6.1 Scenario 1: egh (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-httpg1_trends.png}
    \label{behfig:egh:r1s1http.png}} 

\subfigure[r6.1 Scenario 1: 4tf (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-deviceg1_trends.png}
    \label{behfig:4tf:r1s1device.png}} 
\subfigure[r6.1 Scenario 1: 4tf (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-fileg1_trends.png}
    \label{behfig:4tf:r1s1file.png}} 
\subfigure[r6.1 Scenario 1: 4tf (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-httpg1_trends.png}
    \label{behfig:4tf:r1s1http.png}} 
    
\subfigure[r6.1 Scenario 1: All in One Model]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/ain1-r1s1g1_trends.png}
    \label{behfigure:ain1:r1s1.png}}
\subfigure[r6.1 Scenario 1: Baseline]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/liu-r1s1g1_trends.png}
    \label{behfigure:liu:r1s1.png}}
\caption{r6.1 Scenario 1}
\end{figure*}

\begin{figure*}
\centering    
\subfigure[r6.1 Scenario 2: Acobe (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-deviceg2_trends.png}
    \label{behfig:acobe:r1s2device.png}} 
\subfigure[r6.1 Scenario 2: Acobe (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-fileg2_trends.png}
    \label{behfig:acobe:r1s2file.png}} 
\subfigure[r6.1 Scenario 2: Acobe (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r1s1-httpg2_trends.png}
    \label{behfig:acobe:r1s2http.png}} 
    
\subfigure[r6.1 Scenario 2: egh (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-deviceg2_trends.png}
    \label{behfig:egh:r1s2device.png}} 
\subfigure[r6.1 Scenario 2: egh (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-fileg2_trends.png}
    \label{behfig:egh:r1s2file.png}} 
\subfigure[r6.1 Scenario 2: egh (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r1s1-httpg2_trends.png}
    \label{behfig:egh:r1s2http.png}}     
    
\subfigure[r6.1 Scenario 2: 4tf (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-deviceg2_trends.png}
    \label{behfig:4tf:r1s2device.png}} 
\subfigure[r6.1 Scenario 2: 4tf (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-fileg2_trends.png}
    \label{behfig:4tf:r1s2file.png}} 
\subfigure[r6.1 Scenario 2: 4tf (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r1s1-httpg2_trends.png}
    \label{behfig:4tf:r1s2http.png}} 

\subfigure[r6.1 Scenario 2: All in One Model]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/ain1-r1s1g2_trends.png}
    \label{behfigure:ain1:r1s2.png}}
\subfigure[r6.1 Scenario 2: Baseline]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/liu-r1s1g2_trends.png}
    \label{behfigure:liu:r1s2.png}}
\caption{r6.1 Scenario 2}
\end{figure*}


\begin{figure*}
\centering
\subfigure[r6.2 Scenario 1: Acobe (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s1-device_trends.png}
    \label{behfig:acobe:r2s1device.png}} 
\subfigure[r6.2 Scenario 1: Acobe (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s1-file_trends.png}
    \label{behfig:acobe:r2s1file.png}} 
\subfigure[r6.2 Scenario 1: Acobe (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s1-http_trends.png}
    \label{behfig:acobe:r2s1http.png}} 
    
\subfigure[r6.2 Scenario 1: egh (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s1-device_trends.png}
    \label{behfig:egh:r2s1device.png}} 
\subfigure[r6.2 Scenario 1: egh (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s1-file_trends.png}
    \label{behfig:egh:r2s1file.png}} 
\subfigure[r6.2 Scenario 1: egh (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s1-http_trends.png}
    \label{behfig:egh:r2s1http.png}} 

\subfigure[r6.2 Scenario 1: 4tf (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s1-device_trends.png}
    \label{behfig:4tf:r2s1device.png}} 
\subfigure[r6.2 Scenario 1: 4tf (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s1-file_trends.png}
    \label{behfig:4tf:r2s1file.png}} 
\subfigure[r6.2 Scenario 1: 4tf (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s1-http_trends.png}
    \label{behfig:4tf:r2s1http.png}} 
    
\subfigure[r6.2 Scenario 1: All in One Model]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/ain1-r2s1_trends.png}
    \label{behfigure:ain1:r2s1.png}}
\subfigure[r6.2 Scenario 1: Baseline]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/liu-r2s1_trends.png}
    \label{behfigure:liu:r2s1.png}}
\caption{r6.2 Scenario 1}    
\end{figure*}

\begin{figure*}
\centering    
\subfigure[r6.2 Scenario 2: Acobe (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s2-device_trends.png}
    \label{behfig:acobe:r2s2device.png}} 
\subfigure[r6.2 Scenario 2: Acobe (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s2-file_trends.png}
    \label{behfig:acobe:r2s2file.png}} 
\subfigure[r6.2 Scenario 2: Acobe (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/acobe-r2s2-http_trends.png}
    \label{behfig:acobe:r2s2http.png}} 
    
\subfigure[r6.2 Scenario 2: egh (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s2-device_trends.png}
    \label{behfig:egh:r2s2device.png}} 
\subfigure[r6.2 Scenario 2: egh (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s2-file_trends.png}
    \label{behfig:egh:r2s2file.png}} 
\subfigure[r6.2 Scenario 2: egh (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/egh-r2s2-http_trends.png}
    \label{behfig:egh:r2s2http.png}}     
    
\subfigure[r6.2 Scenario 2: 4tf (Device)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s2-device_trends.png}
    \label{behfig:4tf:r2s2device.png}} 
\subfigure[r6.2 Scenario 2: 4tf (File Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s2-file_trends.png}
    \label{behfig:4tf:r2s2file.png}} 
\subfigure[r6.2 Scenario 2: 4tf (Http Accesses)]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/4tf-r2s2-http_trends.png}
    \label{behfig:4tf:r2s2http.png}} 

\subfigure[r6.2 Scenario 2: All in One Model]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/ain1-r2s2_trends.png}
    \label{behfigure:ain1:r2s2.png}}
\subfigure[r6.2 Scenario 2: Baseline]{
    \includegraphics[width=0.32\textwidth]
    {behfigures/liu-r2s2_trends.png}
    \label{behfigure:liu:r2s2.png}}
\caption{r6.2 Scenario 2}
\end{figure*}



==> trash.tex <==
\subsection{Enterprise Security Protection}
Existing commercialized enterprise-level entity protection includes IBM QRadar SIEM, Symantec Endpoint Protection, Microsoft Windows Defender, and many others.  Most of them heavily depend on incident signatures and anomalous behaviors; however, there are several drawbacks and requirements before they can perfectly identify compromise entities.  Most of them require endpoint software installation, which could be impossible if an enterprise establishes a troublesome bring-your-own-device regulation or culture~\cite{byod1, byod2}

However, most of them are majorly depend on rules, signatures, and heuristics; hence, they require extremely heavy efforts on monitoring risks and tuning parameters for different deployment scenario.  What is worse, most of them require endpoint software installation, which could be impossible if an enterprise establishes a troublesome bring-your-own-device regulation or culture.


Existing commercialized enterprise-level entity protection includes IBM QRadar SIEM, Symantec Endpoint Protection, Microsoft Windows Defender, and many others.  Most of them heavily depend on incident signatures and anomalous behaviors; however, there are several drawbacks and requirements before they can perfectly identify compromise entities.  

Signature-based protection aims to find incidents by finding known malicious pattern or malicious attributes.  

Hence, signature-based protection can only identify identify known incidents, and its accuracy is subjected to effectiveness of available signatures (in other words, high false-negative rate on unknown attacks).  Behavior-based protection, on the other hand, aims to find compromise based on anomalous scores or risk scores that are derived by how much a behavior deviates from usual behaviors.  Hence, behavior-based protection can only work with scenario where each entity always has consistent behaviors, and whenever there is any environmental change (including system updates, network outage, new services) or rare-but-benign signal (including configuring tasks, changing passwords, logon from foreign because of travel) it will raise a false alarm (in other words, high false-positive rate).  To reduce the amount of false positives, most behavior-based protection requires security experts to tune and monitor based on different scenarios.  Last but not least, most of the existing tools require endpoint software installation, which may not always be applicable. 

\begin{enumerate}
\setlength\itemsep{0em}
\item \textbf{Completeness:} Endpoints are often not protected or audited, especially when an enterprise establishes a BYOD culture.  Unprotected endpoints may create new attack surface, and security team may not be aware of suspicious activities due to the lack of audit logs from endpoint devices.
\item \textbf{Interpretability:} An attack can incurs anomalous logs on different entities (e.g., both user and service) and different behaviors (e.g., process executions, file accesses, and network traffics); moreover, audit logs are often composed as sequences of independent events with complex text fields rather than dependent numeric values.  Furthermore, a persistent attack can effect different log types in different ways across multiple dates.  Hence, the resulting log of an attack is multi-sourced, multi-dimensional, and long-lasted.  The challenge is how we can interpret audit logs in a way that we can identify such attack patterns.
\item \textbf{Scalabilty:} In an enterprise of 1.8K entities, 1.5K hosts (servers and endpoints), and 26 Windows servers with SIEM service, one can expect around 70M records of Windows events (from SIEM service) and 20M records of HTTP traffics (including internal, inbound, and outbound traffics) on a working day.  It is difficult for a security team to filter or monitor suspicious activities thoroughly in a timely manner. 
\item \textbf{False Alarms:} An alarm is a set of anomalous signals that needs investigation.  However, there are a few rare-but-benign signals that can cause false alarms, such as signal that results from rare activities due to environmental change (e.g., system update or network outage) or locale change (e.g., holidays or make-up days).  False alarms will overwhelm security team if the amount is not contained.
\end{enumerate}



\begin{table}[]
\centering
\begin{tabular}{| p{1.5cm} | p{6cm} |} \hline
Symbols & Description \\ \hline \hline
$P$, $\mathbb{g}$ & 
    $P_i$ is a behavioral profile configured to have granularity $\mathbb{g}_i$ on objects.  \\ \hline 
$H$, $e$, $\ell$, $\tau$ & 
    $H$ is a sequence of events $e_i=(\ell_i, \tau_i)$, where $\ell_i$ is a label and $\tau_i$ is a timestamp.  \\ \hline
$D$, $d$, $w$ &
    $D_i$ represents a day with $w$ duration windows, from $d_{i,0}$ (starts at 6 am) to $d_{i, w-1}$ (ends by 6 am).  \\ \hline
$\sigma$, $f$, $\epsilon$ & 
    $\sigma_{f,d}$ is a behavioral deviation measurement of a feature $f$ during a duration $d$, and is bounded by $|\sigma_{f,d}| \leq \epsilon$.  \\ \hline 
$\Delta$, $\delta$, $\omega$ &
    $\Delta$ is a deviation matrix which consists of $\omega$ deviation vectors, from $\delta_0$ to $\delta_{\omega-1}$, where $\delta_i=\{\sigma_{f,d}| \forall f, \forall d \in D_i\}$ is a deviation vector that consists of behavioral deviation measurements $\sigma_{f,d}$ on $D_i$.  \\ \hline
\end{tabular}
\caption{Summary of Notations}
\label{anomtab:notation}
\end{table}


Our solution is based on two observations.  Our first observation is that a recently compromised entity may act differently compared to its past.  For example, a compromise could incurs anomalous activities including communication with a command-and-control (C\&C) server, downloading a malicious executable that modifies registry, and probing file system for profitable information.  In this scenario, one would observe anomalous traffics to a C\&C server, anomalous executions of unrecognized executable, anomalous modification upon registry values, and anomalous file accesses and directory traversals.  These activities are not what we would expect from a user's behavioral profile, and we say these activities are behavioral deviations that deviate from a user's profile.  However, simply applying anomaly detection methods (that identify behavioral deviation) could be problematic, as not every deviated activities are suspicious.  Take environmental change as an example, one could expect unrecognized traffics due to new services, unrecognized executable due to software update, or massive amount of repeating queries (retries) due to network outage.  

Recall that we face the following challenges: completeness, interpretability, scalability, and false alarms.  To resolve completeness, we inference user behaviors based on logs gathered from heterogeneous sources (including edge routers, web proxies, and selective servers).  To resolve interpretability, for each user we build multiple behavioral profiles that capture users' normal behaviors and identify behavioral deviation.  To resolve scalability, we propose a behavioral heatmap representation for behavioral deviation across multiple profiles and multiple dates.  To reduce false alarms, in addition to individual behavioral deviation, we embed group behavioral deviation into the behavioral heatmaps in order to capture environmental change and locale change.  

Each event described in $P_1$ to $P_6$ is defined as $e_i=(\ell_i, \tau_i)$, where $\ell_i$ is the coarse-grained label we composed, and $\tau_i$ is a timestamp that indicates when in a day $e_i$ happened; for example, $\tau_i=0$ indicates the beginning of a day (at 12:00 am), and $\tau_i=1439/1440$ indicates the end of a day (at 11:59 pm).  Recall that we build behavior profiles based on history events in order to check whether a sequence of events $H=\{e_0, \dots, e_i\}$ deviates from a user's history.  Hence, for each predictable profile, we build a prediction model (Fig.~\ref{behfig:rnn.pdf}) that takes a sequence of history events $\{e_0,\dots,e_j | 0 \leq j < i\}$ as inputs and generates multi-class prediction probabilities for $e_{j+1}$, and we say a prediction hits if $\ell_{j+1}$ is one of the top half of the predictions sorted by probabilities; otherwise miss.  Our prediction model is similar to the one in Deeplog~\cite{deeplog}; the differences between our approach and Deeplog include that we use bidirectional LSTM RNN (to capture bidirectional dependencies among events), we also consider daily timestamp, and we define hits as top-half (instead of top-9) predictions.   

We aim to identify compromised entities in an enterprise by analyzing audit logs from servers, however, with the constraint of not having information about endpoint devices.  We define an entity as a subject that can be a user, an admin, or a service, specified by one or multiple unique subject name or unique security identifier (SID) across an enterprise.  For example, a user entity can be specified by a unique user account (e.g., user), an email account (e.g., user@enterprise.com), a computer account (e.g., pc-user\$, and a domain account (e.g., ENT\textbackslash user).  We propose an approach that profiles user behaviors, and uses the profiles in finding suspicious entities and time periods that need investigation.  


TODO: Fig.~\ref{behfig:overview.pdf} depicts the overall workflow: we gather heterogeneous audit logs from multiple sources (e.g., windows events, dns, web proxy), for each user we build multiple behavioral profiles $P_1$-$P_6$, for each day $D_i$ we calculate a behavioral deviation vector $\delta_i$, by concatenating several $\delta_i$ we get a deviation matrix $\Delta$, and lastly we check whether $\Delta$ is anomalous with an anomaly-detection model.  Table~\ref{anomtab:notation} summarizes our notations.  In this section, we will focus on how we build behavioral profiles and how we build an anomaly-detection model.  We will not focus on log retrieve, but we will use Windows security-log event-id (eid) as examples to show what we gather.  We split our six profiles into two categories: predictable profiles and statistical profiles.


\begin{itemize}
\setlength\itemsep{0em}
\item \textbf{Deviation Vector:}  $\delta_i=\{\sigma_{f,d} | \forall f, \forall d \in D_i \}$ is a deviation vector for day $D_i$, where $|\sigma_{f,d}| \leq \epsilon$.
\item \textbf{Deviation Matrix:} $\Delta$ is a deviation matrix which consists of $\omega$ deviation vectors, from $\delta_0$ to $\delta_{\omega-1}$, where $\omega$ is the window-size of history in terms of days.
\item \textbf{Behavioral Heatmap:} A behavioral heatmap is a pair of deviation matrices $(\Delta_\mu, \Delta_u)$, where $\Delta_\mu$ is the deviation matrix for a group of entities $\mu$, and $\Delta_u$ is the deviation matrix for a entity $u \in \mu$.  The behavioral heatmap observed at $D_i$ will have $D_i$ as the last day.
\end{itemize}

Fig.~\ref{behfig:compound.png} is an example of a behavioral heatmap, where $w=2$ (i.e., working hours from 6 am to 6 pm, and off hours from 6 pm to 6 am).  For presentation purpose, we split deviation matrices into two heatmap rows ($\Delta_\mu$ on the top and $\Delta_u$ at the bottom) and two heatmap columns (working hours on the left and off hours on the right), in which each pixel represents $\sigma_{f,d_{i,j}}$ for feature $f$ by rows and day $D_i$ by columns (red color indicates positive deviation, white indicates negative, and black indicates no deviation). Fig.~\ref{behfig:compound.png} captures individual behavioral deviation of a compromised user who triggered a ransomware on Feb 2nd, and we can see from the heatmaps that there are deviation in logon profile, command-execution profile, and outbound-flow profile (more details in our attack-case study in Sec.~\ref{anomsec:attack}).  Fig.~\ref{behfig:compound.png} also captures group behavior deviation, and we can see that there are slightly more activities on weekdays and less activities on weekends.


We processes activities day-by-day and period-by-period, as there is deviation correlation among a group of entities during different time period in a day.  We present a day $D_i$ with $w$ duration windows, from $d_{i,0}$ (starts at 6 am) to $d_{i, w-1}$ (ends by 6 am); note that we shift a day by six hours just to align working hours (first-half of $D_i$) and off hours (second-half of $D_i$).  For each duration window $d_{i,j}$, we derive our deviation measurement $\sigma_{f,d_{i,j}}$ for feature $f$, and we use $f(d_{i,j})$ to denote the actual numeric observation of feature during $d_{i,j}$.  We normalize $\sigma_{f,d_{i,j}}$ as shown in Eq.~\ref{anomeq:deviation_measurement}, however bounded within the range $-\epsilon \leq \sigma_{f,d} \leq \epsilon$.  The reason of normalizing $\sigma_{f,d_{i,j}}$ is that each entity may have profiles that are more or less chaotic than the other entities.  For example, an admin entity often has more activities in configuration profile and command-execution profile than the other non-admin entities, whereas a user entity often has more random activities in intranet-flow profile and outbound-flow profile than admin entities and service entities.  Moreover, an IT user could have more random outbound-flow activities at different moment than a non-IT user who has a strict working schedule.  Hence, we normalize our deviation measurement $\sigma_{f,d_{i,j}}$ so that we measure only on how deviated $d_{i,j}$ is compared to the history $d_{k,j}$, where $\omega \leq k < i$, and $\omega$ is the window-size of history in days.  We bound $\sigma_{f,d_{i,j}}$ by $\epsilon$ (e.g., $\epsilon=3$), because it is equivalently anomalous when $\sigma_{f, d_{i,j}} \geq \epsilon$.
